Robust Dynamic Radiance Fields

Dynamic radiance field reconstruction methods aim to model the time-varying structure and appearance of a dynamic scene. Existing methods, however, assume that accurate camera poses can be reliably estimated by Structure from Motion (SfM) algorithms. These methods, thus, are unreliable as SfM algorithms often fail or produce erroneous poses on challenging videos with highly dynamic objects, poorly textured surfaces, and rotating camera motion. We address this robustness issue by jointly estimating the static and dynamic radiance fields along with the camera parameters (poses and focal length). We demonstrate the robustness of our approach via extensive quantitative and qualitative experiments. Our results show favorable performance over the state-of-the-art dynamic view synthesis methods.

==> figures/dynamic_losses.tex <==
\begin{figure}[]
\centering
\includegraphics[width=1.0\columnwidth]{figures/dynamic-crop.pdf}
\caption{\textbf{Training losses for the dynamic radiance field reconstruction.}}
\label{fig:dynamic_losses}
\end{figure}

==> figures/static_losses.tex <==
\begin{figure}[]
\centering
\includegraphics[width=1.0\columnwidth]{figures/static-crop.pdf}
\caption{\textbf{Training losses for the static radiance field reconstruction and poses estimation.}}
\label{fig:static_losses}
\end{figure}

==> figures/view_direction.tex <==
\begin{figure}[]
\centering
\includegraphics[width=1.0\columnwidth]{figures/view_direction-crop.pdf}
\caption{\textbf{Late viewing direction fusion.}~\yulunliu{This figure is pretty much the same as the top of Fig 2. Remove?}}\hy{yeah seems redundant}
\label{fig:view_direction}
\end{figure}

==> setup/graphicspath.tex <==
\graphicspath{{figures}, {examples}}


==> setup/package.tex <==
% Fix "undefined control sequence \Everyshipout".
% \usepackage{everyshi}

% Figures
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{float}
\usepackage[justification=raggedright]{caption}	% makes captions ragged right - thanks to Bryce Lobdell
\usepackage{lscape}                                         % Useful for wide tables or figures.
\usepackage{wrapfig}

% Algorithm
\usepackage[lined,ruled,linesnumbered]{algorithm2e}
\usepackage{animate} %% convert frames to video

% Table and list
\usepackage{booktabs}                   % Publication quality tables
\usepackage{multirow}

\usepackage{makecell}

\usepackage{paralist}
\usepackage{enumitem}
\setlist[enumerate]{itemsep=0mm}

% Math
\usepackage{bm}                          % Make bold, italic math symbols
\usepackage{epsfig}                      % for figures
\usepackage{graphicx}                  % another package that works for figures
\usepackage{times}
\usepackage{mathptmx}
\usepackage{mathtools}
\usepackage{amssymb,amsmath}   % Short math guide for LaTeX ftp://ftp.ams.org/pub/tex/doc/amsmath/short-math-guide.pdf

% Fonts
\usepackage{units}
\usepackage{color}

% Comments
\usepackage{comment}

% Hyperlinks
\usepackage{url}  % Hyphenation of URLs.
%\usepackage[pagebackref=true,breaklinks=true,letterpaper=true,pagebackref=true,colorlinks,bookmarks=false]{hyperref}
\usepackage[pagebackref,breaklinks,colorlinks,linkcolor=blue,citecolor=blue,urlcolor=blue,bookmarks=false]{hyperref}
% \usepackage{authblk}
% \usepackage{slashbox}
\usepackage{xspace}
\usepackage[table]{xcolor}
\usepackage{setspace}
\usepackage{grfext}
\PrependGraphicsExtensions*{.jpg,.png,.PNG}

\usepackage{gensymb}
% \usepackage{emoji}

% \usepackage{times,color}
% \usepackage{parskip}
% %\usepackage{epsfig}
% %\usepackage{psfig}
% %\usepackage[pdftex]{graphicx} % new acmsiggraph.cls
% \usepackage{ifthen}
% %\usepackage[draft]{hyperref} % new acmsiggraph.cls
% \usepackage{float}
% \usepackage{alltt}
% \usepackage{mathenv}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{amsthm}
% %\usepackage{rotating}
% \usepackage{newlfont} % for Box
% %\usepackage{ulem}
% \usepackage{floatflt}
% \usepackage{wrapfig}
% \usepackage{fixltx2e}
% \usepackage{subfig} % for subfloat
% \usepackage{multirow}
% \usepackage{cleveref}
% \usepackage{algorithmic}
% \usepackage{CJKutf8} % Chinese


==> setup/symbols.tex <==
% Define math symbols that appear in the texts

\def\xi{\mathbf{x}_i}
\def\yi{\mathbf{y}_i}

